ALERT: Zero-shot LLM Jailbreak Detection via Internal Discrepancy Amplification

Despite rich safety alignment strategies, large language models (LLMs) remain highly susceptible to jailbreak attacks, which compromise safety guardrails and pose serious security risks. Existing detection methods mainly detect jailbreak status relying on jailbreak templates present in the training data. However, few studies address the more realistic and challenging zero-shot jailbreak detection setting, where no jailbreak templates are available during training. This setting better reflects real-world scenarios where new attacks continually emerge and evolve. To address this challenge, we propose a layer-wise, module-wise, and token-wise amplification framework that progressively magnifies internal feature discrepancies between benign and jailbreak prompts. We uncover safety-relevant layers, identify specific modules that inherently encode zero-shot discriminative signals, and localize informative safety tokens. Building upon these insights, we introduce ALERT (Amplification-based Jailbreak Detector), an efficient and effective zero-shot jailbreak detector that introduces two independent yet complementary classifiers on amplified representations. Extensive experiments on three safety benchmarks demonstrate that ALERT achieves consistently strong zero-shot detection performance. Specifically, (i) across all datasets and attack strategies, ALERT reliably ranks among the top two methods, and (ii) it outperforms the second-best baseline by at least 10% in average Accuracy and F1-score, and sometimes by up to 40%.

==> Sections/checklist.tex <==
% (Optional) If you don't already have it:
% \newcommand{\mtd}{ALERT}
\section{Additional Discussion and Disclosure}
\subsection{Potential Risks}
We have carefully considered the potential risks associated with this work.
Since \mtd\ is designed as a \emph{jailbreak defense} method that aims to improve the safety and robustness of large language models against malicious prompt manipulation, it does not introduce obvious new risks or misuse scenarios.

Our method does not generate new content, modify user prompts, or amplify harmful instructions.
Instead, it operates as a lightweight detector that analyzes internal model representations to identify jailbreak attempts and can be integrated as a safety filter prior to model deployment.
As such, its intended use is purely protective.

% The primary limitations of this work are practical rather than ethical: \mtd\ requires access to intermediate model activations and may therefore be inapplicable in strictly black-box API settings.
% Additionally, as with any automated safety system, imperfect detection may lead to false positives or false negatives, which should be carefully managed in real-world deployments.

Overall, we believe that this work poses minimal risk and is aligned with the broader goal of enhancing the safe and responsible use of large language models.

\subsection{Use Or Create Scientific Artifacts}
Our work is built on established public safety benchmarks, standard jailbreak attack methods, and open-weight LLMs.
For evaluation, we use three widely adopted jailbreak/safety benchmarks: {AdvBench}, {XSTest}, and {StrongREJECT}.
We do not modify the original harmful prompts in these datasets.

In addition, our evaluation protocol constructs two derived artifacts:
(i) a benign counterpart for each harmful prompt (structurally similar but with benign intent), and
(ii) jailbreak prompts generated from harmful prompts using representative jailbreak attacks (e.g., AutoDAN, Adaptive Attack, CodeChameleon).
We will release the codebase and constructed dataset upon publication to facilitate reproducibility and future research.

\subsubsection{Cite Creators Of Artifacts}
All external artifacts are properly credited to their original publications and repositories.
Specifically, the benchmarks {AdvBench}, {XSTest}, and {StrongREJECT} are cited to their respective papers.
The jailbreak attacks (AutoDAN, Adaptive Attack, CodeChameleon) and the evaluated LLM backbones (Llama~3 8B, Mistral 7B, Vicuna-v1.5 8B) are referenced to their official publications or model releases.

\subsubsection{Discuss The License For Artifacts}
We comply with the licenses and usage terms of all artifacts used in this work.
Each dataset and model is used for research purposes under its corresponding license/terms.
Our own code will be released under a compatible open-source license.

\subsubsection{Artifact Use Consistent With Intended Use}
We confirm that our use of the datasets, attacks, and models is consistent with their intended research purpose:
the safety benchmarks are designed to evaluate harmful intent and refusal behavior, and the jailbreak attacks are designed to test robustness against safety circumvention. Both align directly with our goal of studying zero-shot jailbreak detection.


\subsubsection{Data Contains Personally Identifying Info Or Offensive Content}

The datasets used in this work do \emph{not} contain personally identifying information (PII) that could be used to name or uniquely identify individual persons.
All prompts are synthetic or generic natural-language instructions that do not reference real individuals, private attributes, or identifiable personal data.

However, by design, these benchmarks contain \emph{offensive, unsafe, or harmful textual content}, as their primary purpose is to evaluate the robustness of large language models against malicious intent and jailbreak attempts.
We do not attempt to sanitize or alter such content, as doing so would undermine the validity of the safety evaluation.

To ensure responsible use, we take the following steps:
(i) all data are sourced from established, publicly available safety benchmarks that are widely used in prior work;
(ii) the data are used strictly for research purposes on safety detection;
and (iii) no new personal data are collected or introduced during dataset construction.
As a result, no anonymization or de-identification procedures are required, while the presence of offensive content is acknowledged and handled within a controlled research context.

\subsubsection{Documentation Of Artifacts}
We provide detailed documentation of the datasets, attack construction, and model settings in the appendix.
In particular, Appendix~\ref{appdix:main_eval_setting} specifies the main evaluation configuration (datasets, attacks, target LLMs), and Appendix~\ref{appdix:benign_generate} documents benign prompt construction and verification.


\subsection{Statistics For Data}
Dataset statistics and evaluation composition are summarized as follows (see Appendix~\ref{appdix:main_eval_setting} for full details).

\subsubsection{AdvBench}
\begin{itemize}[noitemsep, topsep=0pt]
  \item Content: harmful behaviors formulated as natural-language instructions.
  \item Size: 520 harmful prompts.
  \item Jailbreak construction: harmful prompts are transformed into jailbreak prompts via AutoDAN, Adaptive Attack, and CodeChameleon.
\end{itemize}

\subsubsection{XSTest}
\begin{itemize}[noitemsep, topsep=0pt]
  \item Content: unsafe prompts designed to test exaggerated safety failures.
  \item Size: 200 harmful/unsafe prompts.
  \item Jailbreak construction: same three attack strategies as above.
\end{itemize}

\subsubsection{StrongREJECT}
\begin{itemize}[noitemsep, topsep=0pt]
  \item Content: prompts with explicit harmful intent that should be rejected by aligned models.
  \item Size: 313 harmful prompts.
  \item Jailbreak construction: same three attack strategies as above.
\end{itemize}

\subsubsection{Derived Benign Set Quality}
We additionally evaluate the benignness of the constructed benign prompts using an LLM-based verifier and adopt a hybrid strategy with manual review for samples flagged as non-benign, to avoid over-reliance on automated judgments.

\subsection{Computational Experiments}\label{sec:app-exp}
All computational experiments in this work are designed to be reproducible, with configuration details provided in Appendix~\ref{tab:main_eval}.

\subsubsection{Model Size And Budget}
We evaluate \mtd\ on three representative LLMs:
\begin{itemize}[noitemsep, topsep=0pt]
    \item Llama~3 (8B)
    \item Mistral (7B)
    \item Vicuna-v1.5 (7B)
\end{itemize}
\mtd\ is a lightweight detector without any heavy computations. Since we only use LLMs during inference, all the experiments could run on a single NVIDIA A100 GPU with 40 GB of memory, and the running time for each experiment setting is less than 4 hours.

\subsubsection{Experimental Setup And Hyperparameters}
We adopt a zero-shot jailbreak detection protocol.
For each dataset, jailbreak prompts are generated from harmful prompts using AutoDAN, Adaptive Attack, and CodeChameleon, and each jailbreak set is mixed with a roughly equal number of benign prompts to form the test set.
We report Accuracy and F1-score.

For \mtd, we employ VIB-based detectors with a two-hidden-layer architecture, train for 15 epochs with learning rate $10^{-4}$, and tune remaining VIB hyperparameters via Optuna (e.g., hidden dimension, latent dimension, $\beta$, and Monte-Carlo samples) as specified in Appendix~\ref{tab:main_eval}.

\subsubsection{Descriptive Statistics}
We report Accuracy (Acc) and F1-score (F1) on the constructed test sets. Higher values indicate better jailbreak detection performance.
After comprehensively evaluating all methods across datasets, attack strategies, and target LLMs, we provided the average Accuracy and F1-score as well.

\subsubsection{Parameters For Packages}
We use Optuna for hyperparameter optimization.
Additional implementation and environment details will be released together with the codebase to ensure full reproducibility.

\subsection{AI Assistants In Research Or Writing}
AI tools are used in two ways in this work:
(1) to improve writing quality (e.g., spelling, grammar, clarity), and
(2) to support dataset construction/verification, where an LLM-based verifier is used to assess whether generated benign counterparts are indeed benign, supplemented by manual review for flagged cases.

